A Fixed-Parameter Linear-Time Algorithm for Maximum Flow in Planar Flow Networks

We pull together previously established graph-theoretical results to produce the algorithm in the paper's title. The glue are three easy elementary lemmas.

==> Figures/splice.tex <==
%% BEGIN splice.tex

\begin{tikzpicture}[>=stealth',shorten >=1pt,auto,node distance=3 cm, 
    scale = .68, transform shape]
\node[state, inner sep=5.3pt] (A) {\LARGE $v_1$};
\node[state] (B) [right of =A] {\LARGE $v_1'$};
\node[state, inner sep=8pt] (C) [right of =B] {\LARGE $v$};
\node[state] (D) [right of =C] {\LARGE $v_2'$};
\node[state, inner sep=5.3pt] (E) [right of =D] {\LARGE $v_2$};
\node[state, inner sep=5pt] (F) [below of =C] {\LARGE $v'$};

\path[->] (A) edge [above] node [align=center] {\LARGE $e_1$} (B) ;
\path[->] (B) edge [above] node [align=center] {\LARGE $e'_1$} (C) ;
\path[->] (C) edge [above] node [align=center] {\LARGE $e'_2$} (D) ;
\path[->] (D) edge [above] node [align=center] {\LARGE $e_2$} (E) ;
\path[->] (B) edge [left] node [align=center] {\LARGE $f_1$} (F) ;
\path[->] (C) edge [left] node [align=center] {\LARGE $f$} (F) ;
\path[->] (D) edge [right] node [align=center] {\LARGE $f_2$} (F) ;

\Hide{
\node[state] (C) [right of =B]               [label=$s_5$\qquad\ ] {};
\node[state,fill=green!30] (D) [above of =C] [label=$s_6$] {$a,b$};
\node[state] (E) [right of =D]               [label=$s_7$] {};
\node[state,fill=green!30] (F) [above of =B] [label=$s_4$] {$a$};
\node[state] (G) [above of =A]               [label=$s_1$] {};
\node[state] (H) [left of =G]                [label=$s_2$] {};
\path[->] (A) edge [above] node [align=center] {$0.6$} (B) 
          (B) edge [above] node [align=center] {$0.4$} (C)
          (C) edge [right]  node [align=center] {$0.2$} (D)
          (D) edge [bend left]  node [align=center] {$1$} (E)
          (E) edge [bend left,above]  node [align=center] {$0.5$} (D)
          (E) edge [below]  node [align=center] {\quad $0.5$} (C)
          (B) edge [right]  node [align=center] {$0.3$} (F)
          (F) edge [loop right] node [align=center]  {$1$} (F)
          (B) edge [loop below] node [align=center]  {$0.3$} (B)
          (C) edge [loop below] node [align=center]  {$0.8$} (C)
          (A) edge [right] node [align=center]  {$0.4$} (G)
          (G) edge [bend right] node [align=center]  {$1$} (H)
(H) edge [bend right] node [align=center]  {$1$} (G) ;
}
\end{tikzpicture}

%% END splice.tex


==> Figures/spliceDDD.tex <==
%% BEGIN splice.tex

\noindent
% \begin{minipage}[b]{.99\linewidth}
%
\begin{tikzpicture}[scale=.3] 
%       \newcommand\EdgeOpacity{[line width=1.2,->-=.7,black,opacity=.98]};
       \newcommand\EdgeOpacity{[line width=1.4,black,opacity=.98]};
       % 15 x 20 grid
       \draw [help lines, dotted] (0, 0) grid (16,4);
       \coordinate (A) at (0,3);
       \coordinate (B) at (4,3);
       \coordinate (C) at (8,3);
       \coordinate (D) at (12,3);
       \coordinate (E) at (16,3);
       \coordinate (F) at (8,0);
        

       \draw \EdgeOpacity (A) -- (B) ;
       \draw \EdgeOpacity (B) -- (C) ;       
       \draw \EdgeOpacity (C) -- (D) ;
       \draw \EdgeOpacity (D) -- (E) ;
       \draw \EdgeOpacity (B) -- (F) ;
       \draw \EdgeOpacity (C) -- (F) ;
       \draw \EdgeOpacity (D) -- (F) ;       

       \node at (A) {$v_1$};
       \node at (B) {$v_1'$};
       \node at (C) {$v$};
       \node at (D) {$v_2'$};
       \node at (E) {$v_2$};
       \node at (F) {$v'$};  
\end{tikzpicture}
\qquad\quad
%% GRAPH 2 SHOW ONLY BOUNDING EDGES

%       \newcommand\EdgeOpacity{[line width=1.2,->-=.7,black,opacity=.98]};
%       \newcommand\EdgeOpacity{[line width=1.4,black,opacity=.98]};
%       \newcommand\EdgeOpacityA{[line width=1.4,dashed,black,opacity=.3]};
       % 15 x 20 grid
%       \draw [help lines, dotted] (0, 0) grid (12,16);


%% END splice.tex

